Leveraging Large Language Models for Automated Proof Synthesis in Rust

Formal verification can provably guarantee the correctness of critical system software, but the high proof burden has long hindered its wide adoption. Recently, Large Language Models (LLMs) have shown success in code analysis and synthesis. In this paper, we present a combination of LLMs and static analysis to synthesize invariants, assertions, and other proof structures for a Rust-based formal verification framework called Verus. In a few-shot setting, LLMs demonstrate impressive logical ability in generating postconditions and loop invariants, especially when analyzing short code snippets. However, LLMs lack the ability to retain and propagate context information, a strength of traditional static analysis. Based on these observations, we developed a prototype based on OpenAI's GPT-4 model. Our prototype decomposes the verification task into multiple smaller ones, iteratively queries GPT-4, and combines its output with lightweight static analysis. We evaluated the prototype with a developer in the automation loop on 20 vector-manipulating programs. The results demonstrate that it significantly reduces human effort in writing entry-level proof code.

==> sections/related.tex <==
\section{Related Works}
\ziqiao{Could someone fill more related works here && add problems in traditional search-based approach?}
There has been lines of works to automate the proof writing \cite{}. They use
heuristics, search algorithms, and machine learning to assist developers in
constructing formal proofs more efficiently..

Due to {xxx}, recent works combine machine learning into the process. From
invariant inference~\cite{code2inv,cln2inv} to tactic-based proof
generation~\cite{yang2019learning,first2023baldur}, ML becames more and more
helpful in this area. Different from those works, we first applied LLM to
synthesize invariants and intermediate assertions. Our work targets on a super
new verification language and thus demonstrate that future verification tools
can be more efficient without sacrificing its usability with the help from
LLM-based automation.

\ziqiao{add problems in traditional search-based approach?}
There has been lines of works to automate the proof writing \cite{}. They use
heuristics, search algorithms, and machine learning to assist developers in
constructing formal proofs more efficiently..

Due to {xxx}, recent works combine machine learning into the process. From
invariant inference~\cite{code2inv,cln2inv} to tactic-based proof
generation~\cite{yang2019learning,first2023baldur}, ML becames more and more
helpful in this area. Different from those works, we first applied LLM to
synthesize invariants and intermediate assertions. Our work targets on a super
new verification language and thus demonstrate that future verification tools
can be more efficient without sacrificing its usability with the help from
LLM-based automation.
